ENOLA: Linear-Space and Low-Overhead Control-Flow Attestation for Microcontroller-based Systems

Control-Flow Attestation (CFA) aims to precisely verify execution paths to a remote verifier. However, existing solutions are fundamentally incompatible with resource-constrained, microcontroller-based systems due to the following reasons: (1) the overhead of transmitting measurement and trace data scales poorly (i.e., often exponentially) with the number of basic blocks or linearly with the length of execution traces, making such approaches impractical even on high-end microprocessor-based systems and entirely infeasible on microcontrollers; (2) cryptographic keys and measurement data are typically stored in memory, rendering them vulnerable to cold boot and memory corruption attacks, which is a serious threat for field-deployed devices; and (3) reliance on software-based measurements, combined with frequent context switches between the Rich Execution Environment (REE) and the Trusted Execution Environment (TEE), introduces significant performance overhead. In this paper, we present ENOLA, a linear-space and low-overhead control-flow attestation solution for microcontroller-based systems. ENOLA achieves linear transmission complexity with basic blocks, guaranteeing its scalability for larger programs. Moreover, ENOLA uses hardware-assisted measurement computation present in off-the-shelf devices, and avoids key storage in memory. ENOLA also allocates general-purpose registers for measurements to thwart memory corruption attacks. ENOLA significantly reduces context switching overhead by eliminating transitions from REE to TEE for backward-edge measurements. We developed the ENOLA compiler using LLVM passes and a custom attestation engine targeting the ARMv8.1-M architecture. Our evaluation shows that ENOLA reduces data transmission overhead by an average of 52x on the Embench, while maintaining performance comparable to (or exceeding) that of existing approaches.

==> Makefile <==
DOC ?= main.tex
DIFF ?= 1c4e32c # The SP submission
PDFLATEX = pdflatex -shell-escape -synctex=1
BIBTEX = bibtex
RERUN = "(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)
IMG_SRCS = $(wildcard figures/*-source.pdf)
IMG_OBJS = $(patsubst %-source.pdf,%.eps,$(IMG_SRCS))

ALL_TEX_FILES = $(shell find . -type f -name '*.tex')
BIB_FILES = $(wildcard *.bib)

.PHONY: pdf clean

pdf: images $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex *.tex $(BIB_FILES) $(IMG_OBJS) $(ALL_TEX_FILES)
	$(eval DOC_BASE := $(GENS)$(shell basename $@ .pdf))
	rm -f $(DOC_BASE).bbl
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep -i "(Reference|Citation).*undefined" $*.log ; true
#	dvips -o $(DOC_BASE).ps -t letter $(DOC_BASE).dvi
#	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $(DOC_BASE).ps

watch:
	make; fswatch -0 `find . -name "*.tex" -o -name "*.bib"` | xargs -0 -n1 make all

diff:
	git-latexdiff $(DIFF) -- --main main.tex --no-view -o diff.pdf --cleanup all --ignore-makefile --latexopt -shell-escape --ignore-latex-errors --bibtex --whole-tree

clean:
	find . -name "*.aux" | xargs rm -f
	find . -name "*.log" | xargs rm -f
	find . -name "*.out" | xargs rm -f
	find . -name "*.cut" | xargs rm -f
	find . -name "*.gz"  | xargs rm -f
	find . -name "*.synctex*" | xargs rm -f
	find . -name "*.upa" | xargs rm -f
	find . -name "*.upb" | xargs rm -f
	@\rm -f \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
        $(DOC:.tex=.lof) \
        $(DOC:.tex=.lot) \
        $(DOC:.tex=.loc) \
        $(DOC:.tex=.lol) \
	$(DOC:.tex=-src.tar.gz)

images: $(IMG_OBJS)

%.eps: %-source.pdf
	pdftops -eps $< $(<:-source.pdf=.eps)

veryclean: clean
	@\rm -f *~ *.log
	@\rm -f figures/*.eps

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)



==> ack.tex <==
% !TEX root = main.tex
%\section*{Acknowledgment}

% We thank Dejun Yang for the discussions on space and time complexity of existing approaches. 
% We thank Xi Tan for helping port the LLVM toolchain to the Cortex-85 CPU. 
% This material is based upon work supported in part by National Science Foundation (NSF) grants (2237238 and 2329704), and a National Centers of Academic Excellence in Cybersecurity grant (H98230-22-1-0307). Any opinions, findings, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of United States Government or any agency thereof.

%\clearpage

==> challenges.tex <==
% !TEX root = main.tex
\section{Challenges}
\label{s:challenge}
\begin{comment}
	

In this section we record the challenges in CFA-with-PAC:
\subsection{Path Explosion problem}
One of the most import challenge for CFA is path explosion if we go for the pre-computed hash process. 
Because of path explosion, its hard to use hash based approach to verify the execution of remote application.
OAT paper proposes a solution with compact string to reconstruct the CFG at verifier side~\cite{sun2020oat}
\qes{We need to figure out which option to take. Do we follow similar solution to OAT or CFLAT?}
\qes{How about verifying control flow with input to a operation? and validating the hash at the end?}
\solution{We need to check the applications in OAT. Every operation is probably based on some input from sensor or user input. If it is we can send the input to the verifier with a signature. The verifier checks the signature and execute the program with the input. CFA checks are }
\subsection{Loops}
Measurement of loops with conditional statements may be different depending on number of executions.
\clfat{From the figure 1, we can see there is if-else condition in the loop.
Below this figure is how C-FLAT handles loop.}
\begin{itemize}
	\item Loops in general needs number of iterations as measurement will change depending of number of iterations.
	\item If-else conditions needs extra handling mechanism.
\end{itemize}

If we output metadata data for loop handling we can use ideas from LO-FAT paper~\cite{dessouky2017fat}.
Figure~\ref{fig:dummy5}~\ref{fig:dummy6}~\ref{fig:dummy4} have high level idea and example code of backward edge difference of loop handling in the paper.
\begin{figure}[h!]
	
	\includegraphics[width = .48\textwidth]{pics/c-loop-diff.png}
	
	\caption{Looping C code to check linking and non linking instructions} 
	\label{fig:dummy5}
	
\end{figure}

\begin{figure}[t!]
	
	\includegraphics[width = .48\textwidth]{pics/loop-diff.png}
	
	\caption{Disassembly to check loop different of C code} 
	\label{fig:dummy6}
	
\end{figure}

\begin{comment}
\begin{figure}[b!]
	
	\includegraphics[width = .48\textwidth]{pics/lo-fat-loop-handling.png}
	
	\caption{Lo-FAT Loop Handling} 
	\label{fig:dummy4}
	
\end{figure}

\subsection{Sub routine calls within Loops}

\subsection{Break statements}
\clfat{From the figure 1, we can see there is if-else condition with break statement in the loop.
	Below this figure is how C-FLAT handles break statements.}
\subsection{Call-return matching}
Call-return matching is an easier challenge. From figure~\ref{fig:dummy3} we can see an example.
Both \verb|N2| and \verb|N3| can call \verb|N4|, but depending on the caller of \verb|N4| it will either go to \verb|N5| or \verb|N6|.
We need to keep track of the caller (\verb|N2| or \verb|N3|) and add the valid path measurement to valid hash measurement database. 
\clfat{From figure 3 we can see the authentication hash H4a or H4b. Both valid measurements consist of valid return address matching with the caller. For example: if adversary follow a path such as N2, N4 and N6, it will result in a invalid measurement.}
\begin{figure}[h!]
	
	\includegraphics[width = .48\textwidth]{pics/cflatLoop.png}
	
	\caption{C-FLAT Loop Handling} 
	\label{fig:dummy1}
	
\end{figure}

\begin{figure}[t!]
	
	\includegraphics[width = .48\textwidth]{pics/cflatBreak.png}
	
	\caption{C-FLAT Break statement Handling} 
	\label{fig:dummy2}
	
\end{figure}

\begin{comment}

\begin{figure}[b!]
	
	\includegraphics[width = .48\textwidth]{pics/cflatCallReturn.png}
	
	\caption{C-FLAT Call return matching Handling} 
	\label{fig:dummy3}
	
\end{figure}
\end{comment}
\subsection{Multi-threaded programs}
\subsection{Reducing Trace size}

\subsection{Interrupt handling}
Interrupts during the execution of a attestation program can be challenging as this will divert the control flow of the program.
We may consider the interrupt service routine as separate programs and produce a trace to indicate interrupt number.

==> scratch.tex <==
% !TEX root = main.tex
\section{TO-DO List}

Timeline: CCS Deadline April 29, 2024

\begin{itemize}
	\item [DONE] Tomal 2/25 Implement indirect branch compare. Updated workflow. We need indirect table in ME.	
	\item Tomal 2/29 Instrumented code in Section 4.4/4.5	
	\item Tomal 3/5 Have an evaluation section draft. Section skeleton. Start evaluation	
	\item [DONE] Ziming 2/23 Blast paragraph.
	\item Ziming 2/29 System and threat model. 
	\item Ziming 2/29 Introduction draft.
	\item [DONE] Ziming 3/1 Think about some theoretical analysis	
\end{itemize}

\section{Notes and Discussion}

\begin{itemize}
	\item \qes{Can we change the design to store log in the normal world? This will reduce the number of domain switches. }
	\solution{We can use an approach like silhouette, where we use MPU to mark a memory region privileged readable+writable and unprivileged read only. All ENOLA trace store instructions remain privileged stores, but other application store instructions are converted to unprivileged store instructions. This way we ensure that only ENOLA instrumented code can write to the log region protected through MPU.}
	\item For indirect branches it should jump to start address of functions. We can have a early detection mechanism in verifier, if an indirect branch does not belong to function start address pool we can conclude that prover is malicious.
	
	\item \qes We need to handle key exchange for Cortex-A and Cortex-M. Depending on the model the key exchange model will be different.
	\solution{EL3 Secure world is used for setting the keys.}
	\item \qes QARMA block cipher family has a Tweak. We need figure out if those are accessible or public. Thus while constructing off line measurement database we can use the value.~\cite{avanzi2017qarma}
	\item \qes In angr what is the difference between static vs dynamic analysis?
	\item \qes For CFLAT example figure 1. How does it detect data oriented attacks? If auth is overwritten it will call privileged function. But its still a valid control flow. \solution{CFLAT does not consider pure data oriented attacks. They claim non-control data attack prevention but their procedure does not bind the data variables in the chain. Their examples are based on data variable that controls a loop and based on the generated has it can figure out if the variable was tempered.} \qes{how can we provide a solution that works for data oriented attacks?} \solution{OAT paper provides data oriented attack prevention with runtime checking for define and use locations of the variables.}
	\item \qes {Can we develop a solution with PAC to prevent data oriented attacks?} 
	\item OAT paper has PROOF OF CONTROL-FLOW VERIFICATION section which can be used in our project.
	\item \ziming{Will our approach simply report whether a control-flow attack occurred? or it can provide information about the actually executed control-flow path?}
	\tomal{Enola reports actual executed control-flow path with trace data.}
	\item \ziming{The limitation of CFLAT is it only cares about app not kernel, not interrupt-aware. How do we extend our system to kernel? Does OAT cover kernel? Is OAT interrupt-aware?}
	\tomal{OAT or CFLAT both are not interrupt aware and does not cover kernel.}
\end{itemize}
